Robotics During a Pandemic: The 2020 NSF CPS Virtual Challenge -- SoilScope, Mars Edition

Remote sample recovery is a rapidly evolving application of Small Unmanned Aircraft Systems (sUAS) for planetary sciences and space exploration. Development of cyber-physical systems (CPS) for autonomous deployment and recovery of sensor probes for sample caching is already in progress with NASA's MARS 2020 mission. To challenge student teams to develop autonomy for sample recovery settings, the 2020 NSF CPS Challenge was positioned around the launch of the MARS 2020 rover and sUAS duo. This paper discusses perception and trajectory planning for sample recovery by sUAS in a simulation environment. Out of a total of five teams that participated, the results of the top two teams have been discussed. The OpenUAV cloud simulation framework deployed on the Cyber-Physical Systems Virtual Organization (CPS-VO) allowed the teams to work remotely over a month during the COVID-19 pandemic to develop and simulate autonomous exploration algorithms. Remote simulation enabled teams across the globe to collaborate in experiments. The two teams approached the task of probe search, probe recovery, and landing on a moving target differently. This paper is a summary of teams' insights and lessons learned, as they chose from a wide range of perception sensors and algorithms.

==> tex/Acknowledgements.tex <==
\section{Acknowledgements}
\label{sec:acknowledgements}
We gratefully acknowledge NSF grant CNS-1521617 for this work.

==> tex/Discussion.tex <==
\section{discussion}
\label{sec:discussion}
% We should cite papers from previous CPS Challenge and talk about the differences in regards to what students learned and what was accomplished
Under normal circumstances, this competition would have taken place outdoors and software would have been tested on real drones and flyable hardware.



==> tex/FutureWork.tex <==
\section{Conclusions and Future Work}
\label{sec:future-work}

In this paper, we presented an sUAS for deployment and recovery of a novel environmental smart probe. The probe design is versatile and lightweight, enabling its use as a pest trap for pest-density monitoring in a farm, as well as other applications such as pathogen collection. The autonomous deployment and recovery of these traps using our sUAS would result in significant time and cost savings while allowing larger quantities of useful data and samples to be collected from the field.

As part of the NSF-sponsored student UAV competition, we performed several successful field trials, including achieving the goal of demonstrating the deployment of a scale-model mosquito trap. While autonomous recovery was successfully tested as a subsystem indoors in a controlled setting, during the field test the module  was disabled due to multiple challenges and time constraints. The successful indoor tests demonstrate that autonomous recovery of such a probe is possible and the next step is to expand this into outdoor environments and test the integration with the full mission controller.

To support these efforts, future work will focus on improving the trap design for increased robustness to field conditions, while at the same time improving the ease of docking and also reducing the trap's aerodynamic footprint as it is in the direct down-wash of the UAV propellers. Likewise, the precision payload pickup and deployment capabilities have applications outside agricultural work. Beyond the obvious UAV package delivery, this precise navigation and control using visual-servoing without MOCAP in an outdoor environment can also be used in other precision aerial manipulation tasks.

==> tex/Introduction.tex <==
\section{Introduction}
\label{sec:intro}
% {\small \emph{1) challenge with insects, sampling and impact 
% 2) Why UAS deployment and recovery is needed 
% 3) Our design goal}}

% Should replace figure still, if we have other pictures of physical sUAS that we may want
\begin{wrapfigure}{R}{0.21\textwidth}
\vspace*{-0.12in}
\centering
\includegraphics[width=0.21\textwidth]{imgs/uav-with-magnet.png}
\caption{\label{fig:uav-booth-orange}Our sUAS in flight during field trials. The cable at the bottom suspends an electro-permanent magnet used for docking with a novel lightweight probe assembly.}
\end{wrapfigure}

%%%%%%%% INTRODUCE SUAS AND ITS APPLICATIONS IN SAMPLING %%%%%%%%%


Small Unpiloted Aircraft Systems (sUAS) are gaining popularity in agricultural and environmental applications. sUAS are used for vegetation mapping, crop stress monitoring, and fruit counting through a suite of onboard sensors \cite{dasCASE2015, das2016}. Furthermore, sUAS has been effectively used in missions to retrieve physical samples for ex-situ analysis. For instance, the aerial collection of water samples and aerobiological sampling in agricultural fields ~\cite{ore2015, schmale2008development}. 

%%%%%%%% INTRODUCE CPS CHALLENGE AND ITS VIRTUAL DIFFICULTY IN COVID-19 %%%%%%%%%
The NSF-sponsored 2020 CPS Challenge is motivated by the plethora of application of sUAS. The intention originally was to create an entirely autonomous system with sUAS to deploy and retrieve a soil probe that could measure various soil properties of the Sonoran Desert. However, during the COVID-19 pandemic, building and testing of the hardware became infeasible. To adapt to these new challenges, the challenge moved to a virtual environment and changed its scope.

%%%%%%%% SPECIFY THE 2 PHASES OF THE COMPETITION %%%%%%%%%
In this work, we present two simulated sUAS capable of autonomously retrieving and deploying a lightweight probe, then autonomously landing on a moving rover. We also address the new challenges faced by the pandemic and how they affected our final solutions. To carry out this mission autonomously, an sUAS needs to possess the following capabilities.


%%%%%%%% CONNECT THE GOAL WITH MARS 2021 MISSION %%%%%%%%%
Inspired by the Mars Perseverance Rover and the Mars Helicopter Ingenuity, the new challenge involves a simulated Martian environment, where teams seek to autonomously retrieve and deploy a soil probe using a sUAS and then return the sUAS to a moving rover. Studies have already been conducted showing the efficacy of operating a sUAS on the surface of Mars for scouting purposes and Ingenuity will test them in practice this year~\cite{grip2017flight,balaram2018mars}. Furthermore, retrieving and testing a diverse set of Mars soil samples is one of Perseverance's main science goals~\cite{mustard2013report}. Therefore, soil sampling and retrieval is of interest to the scientific community, and using an sUAS to retrieve samples is not only feasible, but could also allow for samples to be retrieved from locations that are hazardous for rover traversal. A future Mars mission where a sUAS is responsible for critical path science goals, such as probe retrieval, is highly likely, and this challenge lays the groundwork for three autonomy solutions to this specific problem.


\renewcommand{\theenumi}{\alph{enumi}}
\begin{itemize}
\item Autonomously navigate to a search location to search for, detect, descend upon, and pick up the soil probe.
\item Autonomously navigate to a drop location, descend, and detach the soil probe.
\item Autonomously return to and land on a moving rover.
\end{itemize}
We make the following key contributions towards developing and simulating the sUAS.
\begin{enumerate}
\item Extensive use of the OpenUAV simulation framework \cite{anand2019openuav}.
\item Extensive use of Docker for remote work \cite{boettiger2015introduction}.
\item Creation of Gazebo environment that utilizes ROS, PX4, and QGC to accurately simulate drone flight.
\item Multiple solutions to a novel problem that are verified and tested in a simulated environment.
\end{enumerate}

%%%%%%%% ACADEMIC AND EDUCATIONAL ASPECTS %%%%%%%%%
Furthermore, use of OpenUAV and Docker has enabled education involving cyber-physical systems to continue, despite the pandemic. These remote tools allowed for the continuation of the CPS challenge and enabled students from different countries to interact and compete with each other, which would not have been possible under normal circumstances.

%%%%%%%% STRUCTURE %%%%%%%%%
This paper follows the methodologies of two different teams and the structure is as follows. In section~\ref{sec:sys-desc}, we describe the simulation environment, followed by a description of our solutions in~\ref{sec:method}. We discuss simulation results in section~\ref{sec:experiments}, followed by a discussion of the pandemic's impact on the results and the overall preferred methodology in section~\ref{sec:discussion}. Finally, we conclude and outline our next steps in section~\ref{sec:future-work}.  



==> tex/LessonsLearned.tex <==
\section{Lessons Learned}

\subsection{Lost UAV, and recovery}

\subsection{Future Applications}



==> tex/Method.tex <==
\section{Competition Description}
\label{sec:sys-desc}
\subsection{System Description}

A combination of two 2.1 GHz 16 core processor, two NVIDIA GeForce RTX 2080ti, 2 TB SSD and, 10 TB HDD forms the hardware framework of our server. The server can support an average of 50 containers running in parallel. The remote sUAS simulation software is based on OpenUAV \cite{schmittle2018openuav}. The core of the simulation is built upon three components -- (i) ROS and gazebo, (ii) PX4 (iii) MAVROS. The ROS framework helps to pass messages between the different process and is used for sensor hardware abstraction. PX4 is an open source flight controller. The MAVROS package acts as a link between the user program and the sUAS. MAVROS links the PX4 controller with the sUAS by converting ROS messages to MAVLink communication protocol.    

\subsection{Containerization}
Containerization is an operating system level virtualization where applications are run in isolated namespace called containers. The docker orchestration tool enables to pack of the software, its libraries, and dependencies into a lightweight container \cite{boettiger2015introduction}. Docker provides a lightweight virtual environment called an image. This environment is shared with the server and eventually with the remote computers by port forwarding. Docker images are prototypes that can be instantiated in each container. Initially, OpenUAV containers only allowed to run multiple simulation scenarios in parallel. Now, each container is an integrated workspace that allows remote software development using SSHFS.  

\subsection{ROS and Gazebo}
ROS and gazebo together make the basic framework of the robotic simulation. ROS is a framework to easily communicate between the robot and ROS nodes through ROS messages \cite{quigley2009ros}. Gazebo is the simulator that comes with a physics engine \cite{koenig2004design}. The MAVlink communication protocol allows the communication between the UAV model in the simulation with the code written by the user. 

 
\subsection{PX4, MAVROS, and QGC}
PX4 is an open-source flight control software for drones and unmanned vehicles. It provides a wide variety of UAV models and capability of flight control. PX4 enables low level rate control and higher level velocity and position control of the UAV. It also provides sensor support, flight logging and the state estimator. 
QGroundControl is a remote flight planning and tracking software. MAVROS is a ROS package which acts as the liaison between PX4, QGC and ROS. 

By aid of software in the loop (SITL) and hardware in the loop (HITL), PX4 and MAVROS reduces the gap between simulation and real testing. The software controlling the real UAV runs in two parts, the higher-level features on an Intel NUC, and the flight controller on the Pixhawk Autopilot. During simulation, the PX4 software in the loop (SITL) takes the role of the PIXhawk Autopilot.  








==> tex/Problem-description.tex <==
% \section{Design Goal}
% \label{sec:problem-description}


==> tex/RelatedWork.tex <==
\section{Related Work}

Jimenez et al. provide a comprehensive survey of computer vision methods for fruit detection \cite{jimenez2000survey} from it's first mention in \cite{schertz1968basic} and \cite{parrish1977pictorial}. A compilation of more recent works describes the current state of the art in fruit detection \cite{syal2013survey}. Previous attempts at automating fruit counting relied on applying computer vision techniques, hand crafted for specific fruit by exploiting their unique attributes such as color \cite{zhao2005tree}\cite{hayashi2005robotic}\cite{hannan2010machine}\cite{seng2009new}\cite{lak2010apple}\cite{arivazhagan2010fruit}\cite{patel2011fruit}\cite{dorj2013computer}\cite{sorghumheads}, texture \cite{zhao2005tree}\cite{arivazhagan2010fruit}\cite{patel2011fruit}\cite{sorghumheads}\cite{guo2013illumination}, shape \cite{parrish1977pictorial}\cite{zhao2005tree}\cite{hannan2010machine}\cite{seng2009new}\cite{lak2010apple}\cite{patel2012automatic} and spatial orientation \cite{patel2011fruit} to separate fruit from background foliage. \textcolor{blue}{The drawbacks of relying on hand-engineered features are that they do not handle occlusion well and do not generalize to a variety of conditions and fruits. Our pipeline addresses these weaknesses by learning these features through deep learning techniques rather than hand-designing them. }

Nuske et al. present a method of grape cluster counting using a radial symmetry transform to identify candidate berry locations followed by a k-Nearest Neighbor learning algorithm for final grape detection \cite{nuske2011yield}. Wang et al. present a method of estimating apple yield using hue thresholding followed by the exploitation of the specular reflectance \cite{pothentexture}  characteristics of controlled artificial illumination to detect fruit \cite{wang2013automated}. \textcolor{blue}{These methods only work well on night time data sets since they control illumination to capture the specular features. Our pipeline generalizes to both night and day time data sets where the environment is not carefully controlled.}

Recent work applying deep learning to agriculture involved the classification of crops from weeds and soil using a fully convolutional network (FCN) \cite{long_shelhamer_fcn} using a large repository of synthetic data \cite{dyrmann2016pixel}. Mortensen et al. used the same modified VGG-16 deep neural network in the identification of crop such as barley and radish \cite{mortensen2016semantic}. \textcolor{blue}{While our pipeline similarly uses the FCN architecture for our blob detector, it goes beyond these approaches by addressing the issue of overlapped fruit and treating fruit counting as a counting problem instead of a simple pixel-wise classification problem. We approach the counting problem using a second neural network and a linear regression to count the number of fruit within each blob detected by the FCN.}

==> tex/Results.tex <==
\section{Experiments}
\label{sec:experiments}
In this section we, discuss the results of the simulated trials for each methodology.

% \begin{figure}[h]
% \centering
% \includegraphics[width=2.5in]{imgs/Figure-8.png}
% \caption{\label{fig:base}Screenshot from SolidWorks of the base.}
% \end{figure}
\subsection{Planet Porters}
\subsection{Drone Trekkers}

\label{sec:field-trial}
%\begin{figure}[htp]
%\centering
%\subfloat[Microsoft Research (MSR) Project Premonition's mosquito trap in the field.~\cite{msr-premonition}]{\includegraphics[height=1.24in]{imgs/HeroLargePremonition-800x550.jpg}\label{fig:msr-trap}}
%\hspace{0.1in}
%\subfloat[Scale-model adaptation of the MSR trap based on our original probe design.]{\includegraphics[height=1.24in]{imgs/trap.png}}
%\caption{{\small The UAS described in this work was used for deployment and recovery of a scale-model of Microsoft Research's Project Premonition mosquito sampling system.}}
%\end{figure}
%\begin{figure}[hb]
%\centering
%\includegraphics[width=3.3in]{imgs/flight.png}
%\caption{\label{fig:flight}UAV in autonomous fight with probe's top funnel suspended through the electro-permanent magnet.}
%\end{figure}

%\begin{figure}[htpb]
%\centering
%\includegraphics[width=3.3in]{imgs/qgc-mission.jpg}
%\caption{\label{fig:qgc-mission}Screenshot of the QGroundControl GCS showing the outdoor mission file. Waypoint 1 is the take-off location, following which the UAV traverses to waypoint 2, then proceeds to waypoint 3, searches for a trap and retrieves it, deploys it at waypoint 4, and flies to waypoint 5 and lands. The distance between waypoint 4 and 5 is around 200 meters.}
%\end{figure}

%\begin{figure}[htpb]
%\centering
%\includegraphics[width=3.3in]{imgs/quad.png}
%\caption{\label{fig:uav}UAV used in the competition as well as top section of mosquito trap used for the trials.}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=3.3in]{imgs/mission-paths-all-teams.jpg}
%\caption{Our sUAS' outdoor trial flight paths at the field trial, in comparison with paths of other teams. Our system demonstrated maximum autonomy in field conditions, carrying out all tasks except trap recovery autonomously. For recovery, the test pilot had to disengage from offboard mode after trap detection, and dock manually. The rest of the mission continued autonomously.}
%\end{figure}




==> tex/Solution.tex <==
\section{Methodology}
\label{sec:method}

% Should probably replace this with the figure from Harish's OpenaUAV paper
\begin{figure}[H]
\centering
\includegraphics[width=3.5in]{imgs/openuav-architecture.jpg}
\caption{\label{fig:uav-booth-orange}
The end-to-end simulation stack is based on the PX4 flight stack, ROS, and Gazebo Simulator. Using the gzweb web-based simulation environment, the simulator could be run on a dedicated server and accessed from any web-enabled device (PC and mobile).}
\end{figure}
%The simulation setup was used for software development, and a rapid-testing pipeline was used to test different subsystems and individual mission segments prior to field tests. The steps in the testing pipeline are shown in Figure~\ref{fig:software-flow}. In this section, we describe the anatomy of a mission. 
The purpose of the NSF CPS 2020 challenge has been to let contestants explore from a range of perception sensors and develop innovative strategies for trajectory planning and state estimation. State estimation of UAV is a unique challenge due to a persistent pitch angle of the aircraft while flying between destinations. Moreover, the jerks due to aggressive change of modes results in noisy state estimation. A robust strategy is to write a controller that compensates for the inaccuracy in the sensory readings due to the pitch of the aircraft and avoids jerk.

In this competition, the simulation environment is the Jerezo crater on Mars, a possible site for the occurrence of traces of life in space. The 3DR Iris Quadcopter is the simulated agent for the competition. The competition is inspired by the recent announcement by NASA \cite{potter2020mars} on the deployment of the rover Perseverance and the helicopter Ingenuity to explore the Jerezo crater. The presence of a thin layer of atmosphere on Mars allows for UAVs to fly on Mars. This can be seen in figure \ref{fig:environment}.

\begin{figure}[H]
\centering
\includegraphics[width=3.5in]{imgs/Mars_Jezero_Screenshot.jpg}
\caption{\label{fig:environment}
The finished simulated environment containing the Mars Jezero texture, the SUV, and the drone.}
\end{figure}

The competition tries to reduce the gap between simulation and reality by emulating the Martian terrain. The high definition graphical openUAV test bed is rendered to containers with OpenGL and TurboVNC.

%(Here we need to explain the portions of the project  that all teams have in common, I'm not sure what those are at the moment)
Due to the requirements of the competition, all teams followed the same general method to solve this problem as shown in the state diagram in figure \ref{fig:software-flow}. Each methodology begins we a search pattern to find the probe. Each team uses a different object detection algorithm to detect the probe. Once the probe is detected, the teams control the descent of the drone to pick up the probe, which is then carried to the deployment destination. Finally, the teams autonomously return the drones to the SUV and land in the trunk using their own methodologies. 

\begin{figure}[htpb]
\centering
% Define block styles
\tikzstyle{decision} = [diamond, draw, fill=blue!20, 
    text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, fill=blue!20, 
    text width=5em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    minimum height=2em]
    
\begin{tikzpicture}[node distance = 2cm, auto]
    % Place nodes
    \node [block] (pattern) {Search Pattern};
    % \node [cloud, left of=init] (expert) {expert};
    % \node [cloud, right of=init] (system) {system};
    \node [block, below of=pattern] (detection) {Probe Detection};
    \node [block, below of=detection](retrieval){Probe Retrieval};
    \node [block, below of=retrieval] (deployment) {Probe Deployment};
    %\node [block, left of=simulation, node distance=3cm] (fix) {Fix issues};
    \node [block, below of=deployment] (return) {Return to SUV};
    \node [block, below of=return] (landing) {Land in SUV};
    % Draw edges
    \path [line] (pattern) -- (detection);
    \path [line] (detection) -- (retrieval);
    \path [line] (retrieval) -- (deployment);
    \path [line] (deployment) -- (return);
    % \path [line] (decide) -| node [near start] {yes} (update);
    \path [line] (return) -- (landing);
    %\path [line] (fix) |- (create);
    %\path [line] (simulation) -- (fix);
    %\path [line] (indoor) -| (fix);
    %\path [line] (outdoor) -| (fix);
    %\path [line] (decide) -- node {no}(stop);
    %\path [line,dashed] (expert) -- (init);
    %\path [line,dashed] (system) -- (init);
    %\path [line,dashed] (system) |- (evaluate);
\end{tikzpicture}
\caption{\label{fig:software-flow}General State Diagram for all Methodologies.}
\end{figure}


\subsection{Team Drone Trekkers}
This solution utilized color and shape recognition for probe detection. Using terrain relative navigation, the drone followed a "lawnmower" pattern to search for the drone. Then, using OpenCV packages the drone detected the probe as a red circle. Following that, the drone used velocity control to descend upon the probe, where a gazebo plug-in was used to attach to the probe model. At this point, the drone took the probe to a pre-determined drop location, where the drone descended and detached the probe.

Next, the drone navigates to the SUV while the SUV starts to move forward. The drone navigates to the estimated position of the SUV. This is accomplished using the GPS location of the SUV, as well as RTAB-map coordinates folded into a Kalman Filter. This should allow for reasonably accurate SUV pose estimation. When the drone hovers above the SUV, it detects the SUV using YOLO implemented through the darknet ros package. As the drone descends, it uses fiducials located in the trunk of the SUV to refine its landing and successfully drop into the trunk.

A major shortcoming of this approach was that RTAB-map did not work when the terrain lost features. Due to the way the simulation environment was constructed, the terrain lost sufficient detail to create a point cloud for RTAB-map to use to deduce location. Therefore, if the SUV traveled too far, the Kalman Filter would stop working and the drone would be unable to follow the SUV. However, this problem would not happen in a real-world environment, as there would be plenty of features from the desert landscape. Therefore, this solution should work in general, but given the constraints of the online-environment, its success is limited in this competition.

\begin{figure}[h]
\centering
\includegraphics[width=3.5in]{imgs/Probe Pick Up.jpg}
\caption{\label{fig:obstacle}Drone Trekkers using color and shape recognition to detect the red probe with their drone. The drone is in the process of using velocity control to descend onto, and pick up, the probe.}
\end{figure}

%The obstacles were made up of several polygons in a 2-dimensional space. After reading these polygons and labeling the world space, takeoff, pickup, drop-off, and landing locations, the algorithm divided each task and created an occlusion map of the region. When creating the map and building the respective nodes and edges, a function was called to verify the validity of the current node. The verification to check whether a node was inside a no-fly zone used the technique of ray casting, checking how many times a ray starting from the point intersects with the edges of the polygon. If the point is outside the polygon, it will intersect with the edges an even number of times, whereas if it's inside, it will intersect with the edges an odd number of times. If the node was found to be inside any of the forbidden zones, the links or edges leading to this node were not created, preventing the UAV from flying to this location.


% Planet Porters should change this image to something from their trial
\begin{figure}[h]
\centering
\includegraphics[width=3.5in]{imgs/drone.png}
\caption{\label{fig:rangers}Planet Porters using an array of sonar sensors to detect and avoid the terrain while lifting the sample probe.}
\end{figure}

%Subsequently, the path planning algorithms were created to generate the respective waypoints for the UAV to follow and reach the desired objectives. Three different methods for finding the shortest path to goal were created. The Breadth First Search algorithm explores the occlusion map equally in all directions. Dijkstra’s Algorithm prioritizes the paths to explore and weights them in order to favor the lower cost paths. Finally, the A* is a variation of the Dijkstra’s Algorithm that implements the distance to the goal as a heuristic for the cost of each path. Despite developing the three options, the A* method was determined to be the best choice for the path planning and waypoint generation due to its improved computational time and efficiency for the solution. The GeoJSON file utilized GPS coordinates of latitude and longitude, whereas for practical reasons, the algorithms utilized UTM coordinates. This change was made because the UTM coordinates create a flat representation of the world and turn it into a grid. Hence, after computing the waypoints for the planned path, a conversion back to GPS coordinates was done. 

\subsection{Team Planet Porters}
The solution involves localization of the probe using colour recognition. Once the camera starts providing feedback, a set-point control loop is applied to bring the drone closer to the probe. This is done by detecting red colour using RGB to HSV conversion methods. The centroid of the contour as well as the area of the red contour is extracted and utilized. The drone docks with the probe as it gets closer than 0.6 units.\linebreak

Throughout the mission, the drone toggles between the navigational safety options. Thus discarding safety if it intends to go near the terrain to either land or deploy/dock the probe. For safe navigation, eight sonar sensors have been installed in eight directions of the drone’s horizontal plane. Doing so will help the drone detect any upcoming terrain hills easily because of its forward tilt angle. As any of the sonars sense an obstruction close by, the drone simply hikes up the altitude , without altering the horizontal velocity.\linebreak

After dropping the probe, the drone tracks the rover through the GPS coordinates. The solution now applies a PID control algorithm that controls the velocity of the drone by using the relative displacement between the drone and the rover as input. The rover velocity, which is taken from the ekf output of the px4 software, is also utilized in controlling the drone.




%\begin{figure}[htpb]
%\centering
%\includegraphics[width=3.4in]{imgs/nodesList.jpg}
%\caption{\label{fig:nodesList}Image: Major nodes concerning the process.}
%\end{figure}
%\begin{wrapfigure}{R}{0.19\textwidth}
%\vspace*{-0.12in}
%\centering
%\includegraphics[width=0.19\textwidth]{imgs/search-pattern.png}
%\caption{\label{fig:search-pattern}Search pattern used to locate the trap at the expected position.}
%\end{wrapfigure}

%\begin{wrapfigure}{R}{0.24\textwidth}
%\vspace*{-0.12in}
%\centering
%\includegraphics[width=0.24\textwidth]{imgs/uav-test-indoors.png}
%\caption{\label{fig:trap-recovery}{\small Autonomous trap retrieval using downward camera imagery (video clip at \url{https://goo.gl/XmsXyv}). Although motion capture system was active for ground-truthing UAS performance, the data was not used for trap recovery.}}
%\end{wrapfigure}
%The UAV flies to the expected position of the trap for pickup. Once above this waypoint, it searches for the trap in the nearby area until it detects the trap using the downward-facing camera. The search pattern used is an expanding square search pattern with 1 meter spacing. This search pattern was used for its simplicity to implement, as each waypoint can be generated using the following simple equation. 
%\[ y(n) = \Bigl\lceil{\frac{n}{4}}\Bigr\rceil (-1)^{\lfloor{\frac{n-1}{2}}\rfloor} \]
%\[ x(n) = y(n-1) \]

%The visualization of this search pattern can be seen in figure \ref{fig:search-pattern}. Once the trap detection algorithm detects the trap using the downward-facing camera, the UAV centers itself directly above the trap. The UAV then lowers itself onto the trap, with the electromagnet making contact with a metal washer on the trap. Once this contact is established, the payload is attached, and the UAV can continue its mission. fig.~\ref{fig:trap-recovery} shows autonomous trap recovery indoors.

% \begin{figure}[h]
% \centering
% % Define block styles
% \tikzstyle{point} = []
% \tikzstyle{line} = [draw, -latex']
% \tikzstyle{cloud} = [draw, ellipse,fill=green!20]
    
% \begin{tikzpicture}[node distance = 1cm, auto]
%     \node[cloud](start) at (0,0) {Start};
%     \draw[thin] (start)  -- (0,1);
%     \draw[thin] (0,1)  -- (1,1);
%     \draw[thin] (1,1)  -- (1,-1);
%     \draw[thin] (1,-1)  -- (-1,-1);
%     \draw[thin] (-1,-1)  -- (-1,2);
%     \draw[thin] (-1,2)  -- (2,2);
%     \draw[thin] (2,2)  -- (2,-2);
%     \draw[thin] (2,-2)  -- (-2,-2);
%     \draw[thin] (-2,-2)  -- (-2,3);
%     \draw[thin] (-2,3)  -- (3,3);
% \end{tikzpicture}


% \end{figure}

%\subsection{Solution 3}
%Once the UAV picks up the trap, it flies to the deployment waypoint by switching from offboard mode back to to mission mode. The mission controller constantly monitors the UAV's distance to the deployment waypoint. As the UAV approaches this waypoint, it  descends to approximately 1 meter above the ground. Once the distance is below a set amount (2 meters), the mission controller deactivates the electro-permanent magnet and releases the payload. This is done by briefly turning on a current to the coil in the electro-permanent magnet that cancels out the magnetic field. 


%\subsection{Solution 3}
%The mission manager executes each of the above algorithms and keeps track of the UAV's progress within the mission. It also automatically switches between different Pixhawk modes, such as mission and offboard mode according to the specific task that needs to be completed. In order to simplify the UAV controller, a stand-alone object-oriented C++ library was written to send commands through MAVROS to the UAV. The locations at which to execute particular tasks were given as waypoints to the Pixhawk flight controller and waypoint indices to the top-level mission controller running on the Intel NUC. For our executing of this mission, the UAV took-off to waypoint 1, picked up the trap at waypoint 2, deployed the trap at waypoint 3 and landed at waypoint 4. The waypoint indices at which of these actions occurred  could be rearranged, thus allowing more complex paths to be taken, such as multiple waypoints between pickup and deployment to avoid a no-fly zone. The full state diagram for the top-level mission controller can be seen in figure \ref{fig:mission-flow}.


==> tex/competition.tex <==
\section{Competition Description}

